Annulus configuration in handlebody-knot exteriors

In contrast to classical knots, the knot type of a genus two handlebody-knot is not determined by its exterior, and it is often a challenging task to distinguish handlebody-knots with homeomorphic exteriors. The present paper considers an invariant (the annulus diagram), defined via Johannson's characteristic submanifold theory and the Koda-Ozawa classification for essential annuli, and demonstrates its capability to distinguish such handlebody-knots; particularly, the annulus diagram is able to differentiate members in the handlebody-knot families given by Motto and Lee-Lee.

==> prelim.tex <==
%%preliminaries:
%%notation
%%2-component links
 
 
Throughout the paper we work in the piecewise linear category.
Given a subpolyhedron $X$ of a $3$-manifold $M$, 
$\mathring{X}$, $\mathfrak{N}(X)$, 
and $\bm X$ denote the interior, 
a regular neighborhood, and
the frontier of $X$ in $M$.
In the event $X$ is a manifold with boundary, 
$\mathring{X}$ could also mean the manifold interior;
the context should make it clear which notion of interior
is being used.
%when the ambient $M$ is clear from the context. 
%(e.g.\ $\opennbhd{X}{M}$).
By the exterior $\Compl X$ of $X$ in $M$, 
we understand the complement of $M-\openrnbhd{X}$ if $X$ has codimension greater than zero, and  
is the closure of $M-X$ otherwise. 
Submanifolds of a manifold $M$ are assumed to be 
proper and in general position except in some obvious cases
where submanifolds are in $\partial M$.  
%intersection of two submanifolds are assumed to be transverse.  
A surface in a $3$-manifold is essential if 
it is incompressible, $\partial$-incompressible, and non-boundary parallel, and an atoroidal (resp.\ a cylindrical) 
$3$-manifold is one that contains 
no essential tori but
some essential annuli.
We denote by $(\sphere,X)$ an embedding 
of $X$ in the oriented $3$-sphere $\sphere$. 
When $X$ is a handlebody, an essential disk in $X$ is also called a \emph{meridian} disk. 
Throughout the paper $\pair$ is a 
handlebody-knot of genus two whose exterior 
is atoroidal and cylindrical.
 
  
%\subsection{Annulus diagram}
\subsection{Characteristic diagram}
Given an atoroidal, irreducible, $\partial$-irreducible  compact oriented $3$-manifold $M$,   
a codimension-zero submanifold $X\subset M$
is admissibly \emph{fibered} if it can either be \emph{Seifert fibered}
with $X\cap \partial M$ consisting of some fibers or be \emph{I-fibered} with 
$X\cap \partial M$ being the two lids of the I-bundle, where a \emph{lid} 
of an I-bundle $\pi:X\rightarrow B$ is a component of the closure of $\partial X-\pi^{-1}(\partial B)$. 
A codimension-zero submanifold $X\subset M$ is \emph{simple} if 
every essential annulus $\annulus\subset X$ not meeting the frontier $\bm X$% of $X$ in $M$ 
is parallel to an annular component $\annulus'$ of $\bm X$; that is, $\annulus$ 
cuts off a submanifold 
%$C$ 
from $X$ that admits an I-bundle structure 
%$\pi:C\rightarrow B$ 
with two lids being $\annulus$
and $\annulus'$, respectively.

By the Johnannson's characteristic submanifold theory,
there exists a surface $\surface\subset M$, unique up to isotopy, 
consisting of essential annuli in $M$ such that  
\begin{enumerate}
\item the closure of each component of the complement $M-\surface$
is either simple or admissibly fibered, and
\item removing any component of $\surface$ 
causes the first condition to fail.
\end{enumerate}

The characteristic diagram $\charM$ is then a graph given by 
assigning to each admissibly fibered (resp.\ simple) component of $M-\surface$ a solid (resp.\ hollow) node, 
and to each component $\annulus$ of $\surface$ 
an edge connecting the node(s)
that correspond to component(s) of $M-\surface$ whose closure(s) contains $\annulus$. 
For instance, the characteristic diagram of the 
exterior of the handlebody-knot $\pairfourone$ 
is \raisebox{-.3\height}{\includegraphics[scale=.1]{peanut}} (see \cite[]{Wan:22p}); 
conversely, any handlebody-knot whose exterior has the characteristic diagram is equivalent to $\pairfourone$ 
\cite[Theorem $1.6$]{Wan:22p}. 
Unlike knots, however, the exterior of a handldebody-knot 
is in general not sufficient 
to distinguish inequivalent handlebody-knots 
\cite{Mott:90}, \cite{LeeLee:12}, \cite{BelPaoWan:20a}.  

\subsection{Types of essential annuli}
Recall that \cite{KodOzaGor:15} and \cite{FunKod:20} classify 
essential annuli in an atoroidal handlebody-knot exterior 
into six types: a type $2$ annulus $\annulus$
is characterized by the property that exactly one component of $\partial \annulus$
bounds a disk $\disk$ in $\HK$; $\annulus$ is said to be of type $2$-$1$ (resp.\ of type $2$-$2$)
if $\disk$ is non-separating (resp.\ separating). 
We use the notation
$\hopf_i$ for a type $2$-$i$ annulus, $i=1,2$, as it is 
also called a Hopf type annulus.
 
A type $3$-$2$ (resp.\ type $3$-$3$) annulus $\annulus$ is characterized by the property
components of $\partial \annulus$ 
do not bound disks in $\HK$ and there exists
an unique, up to isotopy, non-separating (resp.\ separating) essential disk $\disk\subset\HK$ 
not meeting $\partial \annulus$.
A type $3$-$2$ annulus $\annulus$ 
can be further classified into two subtypes: 
if $\annulus$ is essential 
in the exterior of the complement $\HK-\openrnbhd{\disk}$,
it is said of type $3$-$2$i and otherwise of type $3$-$2$ii. 
Furthermore, since $\annulus$ 
cuts a solid torus $V$ off from $\Compl\HK$, 
we define the slope of $\annulus$ to be 
the slope of $\partial \annulus$ 
with respect to $(\sphere, V)$,
and denote by $\knot_\ast(r)$ a type $3$-$2\ast$ annulus with a slope of $r$, $\ast=1,2$; note that 
the essentiality of $\annulus$ implies $r$ is neither integral nor $\infty$.


 
Similarly, for a type $3$-$3$ annulus $\annulus$, 
let $l_1,l_2$ be components of $\partial\annulus$.
Then the unique separating disk $\disk$ cuts $\HK$ into two solid tori $V_1,V_2$ with $l_i\subset \partial V_i$, $i=1,2$. 
The slope pair of $\annulus$ is then an unordered 
pair $(r,s)$
of rational numbers given by the slopes of $l_i$ with respect to $(\sphere, V_i)$, $i=1,2$. 
Denote by $\link(r,s)$ a type $3$-$3$ annulus with a slope pair of $(r,s)$; 
note that by \cite{Wan:23}, 
$(r,s)$ is either of the form $(\frac{p}{q},\frac{q}{p})$, $pq\neq 0$ or of the form $(\frac{p}{q},pq)$, $q \neq 0$, where $p,q\in\mathbb{Z}$.


A type $4$-$1$ annulus is characterized by the property that
components of $\partial \annulus$ bound no disks in $\HK$ and there exist no essential disks
in $\HK$ disjoint from $\partial \annulus$. 
Note that $\annulus$ is necessarily separating 
and in addition, it cuts off a solid torus, whose core in $\sphere$ is an Eudave-Mu\~noz knot; 
the notation $\EM$ is reserved for such an annulus. 

Given an atoroidal handlebody-knot $\pair$, 
the annulus diagram $\anndiag$ is the characteristic diagram $\charE$ of $\Compl\HK$
together with a labeling that assigns to each edge $\hopf_i, \knot_i(r), \link(r,s)$ or $\EM$, depending
on the type of the annulus it represents, where $i=1,2$ and $r,s\in\mathbb{Q}$.

\subsection{Examples}

\begin{figure}[t]
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{hk5_1}
\caption{$\pairfiveone$.}
\label{fig:hkfiveone}
\end{subfigure}
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{hk5_1ann}
\caption{Annulus in $\Compl {5_1}$.}
\label{fig:annuli_ext_fiveone}
\end{subfigure}
%\end{figure}
%
%\begin{figure}[h]
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{hk6_1}
\caption{$\pairsixone$.}
\label{fig:hksixone}
\end{subfigure}
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{hk6_1ann}
\caption{Annuli in $\Compl {6_1}$.}
\label{fig:annuli_ext_sixone}
\end{subfigure}
\caption{Handlebody-knots in the knot table \cite{IshKisMorSuz:12}.}
\end{figure}
 
  

Consider first the handlebody-knot $\pairfiveone$ (Fig.\ \ref{fig:hkfiveone}) in the handlebody-knot table \cite[table $1$]{IshKisMorSuz:12}. It admits a type $2$-$1$ annulus $\annulus$ (see Fig.\ \ref{fig:annuli_ext_fiveone}), which is the unique annulus by \cite[Theorem $1.5$]{Wan:22p}, so its annulus diagram is  
\raisebox{-.4\height}{\includegraphics[scale=.13]{hkfiveone_ann_diag}}.

Similarly, we can determine the annulus diagram of the handlebody-knot $\pairsixone$ (Fig.\ \ref{fig:hksixone}) in \cite[Table $1$]{IshKisMorSuz:12}. 
%\includegraphics[scale=•]{•},
Since $\pairsixone$ admits a type $2$-$2$ annulus $\annulus_1$, by \cite[Theorem $1.5$]{Wan:22p},
the annulus diagram is one of the diagrams in Fig.\ \ref{fig:typetwotwo_ann_diags}. 
\begin{figure}[t]
\begin{subfigure}{.3\linewidth}
\center
\includegraphics[scale=.13]{typetwotwo_diagram1}
\end{subfigure}
\begin{subfigure}{.35\linewidth}
\center
\includegraphics[scale=.13]{typetwotwo_diagram2}   
\hspace*{.1em}
\raisebox{2.5\height}{{\tiny, $r\in \mathbb{Q}$, $i=1,2$}}
\end{subfigure}
\begin{subfigure}{.3\linewidth}
\center
\includegraphics[scale=.13]{typetwotwo_diagram3}
\end{subfigure}
\caption{Annulus diagrams.}
\label{fig:typetwotwo_ann_diags}
\end{figure} 
\noindent
Observe now that $\Compl{6_1}$ admits 
a M\"obius band $\mobius$ in 
Fig.\ \ref{fig:annuli_ext_sixone}, 
and there exists a separating disk $\disk_s$
disjoint from $\partial \mobius$. 
Since the core of the component $V$ 
of $\HK-\openrnbhd{\disk_s}$ 
containing $\partial \mobius$ is a trivial knot,
the frontier of a regular neighborhood 
of $\mobius$ is a type $3$-$2$ii
annulus $\annulus_2$ and hence its annulus diagram is the second one in Fig.\ \ref{fig:typetwotwo_ann_diags}. 
The boundary slope of $\mobius$ with respect to
$(\sphere,V)$ is $2$, so the annulus diagram of $\pairsixone$ is \raisebox{-.4\height}{\includegraphics[scale=.13]{hksixone_ann_diag}}.

     
Lastly, we consider the handlebody-knot $\pairfivetwo$ (Fig.\ \ref{fig:hkfivetwo}) in \cite[Table $1$]{IshKisMorSuz:12}. Observe first that it admits a type $3$-$3$ annulus $\annulus$
and a M\"obius band $\mobius$ as shown in Figs.\ \ref{fig:annuli_ext_fivetwo} and \ref{fig:Mobius_ext_fivetwo}.
Note that the frontier of a regular neighborhood of $\mobius$ 
in $\Compl\HK$ is a type $3$-$2$ annulus $\annulus_m$ since there exists a non-separating disk $\disk\subset 5_2$ 
disjoint from $\partial \mobius$. Since the core of the solid torus $V:=\HK-\openrnbhd{\disk}$ is 
a trivial knot in $\sphere$, $\annulus_m$ is of type $3$-$2$ii.

\begin{figure}[t]
\begin{subfigure}{.25\linewidth}
\center
\includegraphics[scale=.08]{hkfivetwo_v1}
\caption{$\pairfivetwo$.}
\label{fig:hkfivetwo}
\end{subfigure}
\begin{subfigure}{.35\linewidth}
\center
\includegraphics[scale=.08]{hk5_2ann}
\caption{Type $3$-$3$ annulus in $\Compl {5_2}$.}
\label{fig:annuli_ext_fivetwo}
\end{subfigure}
\begin{subfigure}{.35\linewidth}
\center
\includegraphics[scale=.08]{hk5_2mobi}
\caption{M\"obius band in $\Compl {5_2}$.}
\label{fig:Mobius_ext_fivetwo}
\end{subfigure}
%\begin{subfigure}{.45\linewidth}
%\center
%\includegraphics[scale=.05]{hk5_2mobi_highlighted}
%\caption{The M\"obius band $M$.}
%\label{fig:mobius_M}
%\end{subfigure}
%\end{figure} 

%\begin{figure}[h]
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{hk5_2intersection}
\caption{$\annulus\cap \mobius$.}
\label{fig:intersection}
\end{subfigure} 
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{hk5_2bundle}
\caption{$I$-bundle structure.}
\label{fig:bundle}
\end{subfigure} 
\caption{$\pairfivetwo$ and $\annulus,\mobius\subset \Compl{5_2}$.}
\end{figure} 
Note that $\annulus$ and $\mobius$ meets at an arc (Fig.\ \ref{fig:intersection}). 
Let $U$ be a regular neighborhood $U$ of $\annulus\cup \mobius$ in $\Compl{5_2}$. Then 
there is an admissible I-bundle structure $U\rightarrow B$, where $B$ is a Klein bottle
with one disk removed (Fig.\ \ref{fig:bundle}). In particular, this implies the characteristic diagram
of $\Compl{5_2}$ is 
\raisebox{-.1\height}{\includegraphics[scale=.2]{char_diag_stick}}, where the annulus $\annulus_c$ 
corresponding to the edge 
is the frontier of $U$ in $\Compl {5_2}$. 
To determine the type of $\annulus_c$, 
we consider the following lemmas.

%%start from here
\begin{lemma}\label{lm:typethreetwoii_generator}
Let $\annulus$ be a type $3$-$2$ii annulus in 
the exterior of 
%a handlebody-knot 
$\pair$. 
Then the image of the homomorphism
$H_1(\annulus)\rightarrow H_1(\Compl\HK)$ is a generator.
\end{lemma}
\begin{proof}
Let $\disk\subset \HK$ be the unique, up to isotopy, non-separating disk disjoint from $\partial \annulus$ and set 
$W:=\HK-\openrnbhd{\disk}$.   
Since $\annulus$ is $\partial$-compressible in 
$\Compl W$, it cobounds a solid torus $U'\Compl W$ with 
the annulus in $\partial W$ cut off 
by $\partial \annulus_c$ that meets $\rnbhd{\disk}$. 
In particular, the induced homomorphism
$H_1(\annulus_c)\rightarrow H_1(U')$ 
is an isomorphism. On the other hand, 
$U$ can be obtained by 
digging a tunnel through $U'$, 
namely $U'=U\cup\rnbhd{\disk}$,
and therefore there is a short exact sequence:
\[0\rightarrow H_2(U',U)\rightarrow H_1(U)\rightarrow H_1(U')\rightarrow 0.\]   
%\begin{equation}\label{eq:generator}
%\text{
The claim thus follows.
\end{proof}

\begin{lemma}\label{lm:typefourone_exclusion}
If 
%a handlebody-knot 
$\pair$ 
admits a type $4$-$1$ annulus $\annulus$, then
every essential annulus disjoint from $\annulus$ is separating.
\end{lemma}
\begin{proof}
Let $V$ be the solid torus cut off by $\annulus$ 
from $\Compl\HK$, 
and $W$ the closure of $\Compl\HK-V$. 
Denote by 
$\annulus'$ the annulus cut off by $\partial \annulus$ 
from $\partial \HK$. Then by the definition of a type $4$-$1$ annulus, the closure $\torus$ 
of $\partial\HK-\annulus'$, 
a torus with two open disks removed, 
is essential in $\Compl V$. 

Now, since no essential disk in $\HK$ disjoint from 
$\annulus$ exists, $\annulus'$ is essential in $\Compl W$.
On the other hand, by the essentiality of $\annulus'$, 
if there exists a non-trivial $\partial$-compressing disk of $\Compl W$, then there exists a non-trivial $\partial$-compressing disk of $\Compl W$ disjoint from $A'$, 
but this contradicts $T$ being essential in $\Compl V$. 
Therefore, $\Compl W$ is $\partial$-irreducible. 
This implies $W$ is $\partial$-reducible, so 
the frontier of the compression body of $W$ is empty, a torus or two tori.
The latter two cases are excluded since $\pair$ is atoroidal. Thus we have shown $W$ is a handlebody of genus two. Applying \cite[Theorem $1.4$]{Prz:83}, 
$\torus$ induces an incompressible torus
$\hat{\torus}$ in the $3$-manifold $\hat{M}$ 
obtained by performing 
Dehn surgery on $V$ along the boundary of 
$\annulus$. Since $\annulus$ is essential in $\Compl\HK$, the boundary slope of $A$ with respect to $(\sphere,V)$ is non-integral. Hence,
by \cite[Lemma $3.14$]{KodOzaGor:15}, 
the core of $V$ is a hyperbolic knot, and therefore an Eudave-Mu\~noz knot by \cite{GorLue:04}. 
In particular, 
there exists an incompressible torus $\torus_0$
that separates $\hat M$ into two Seifert fiber spaces over the disk with two exceptional fibers \cite{Eud:97}, \cite{Eud:20}. 
Note that $\hat M$ 
is itself not Seifert-fibered by \cite{BoyZha:98},
being obtained by an non-integral Dehn surgery on $(\sphere,V)$. Isotope $\torus_0$ so that the number of 
components in 
$\hat \torus \cap \torus_0$ is minimized. Then 
the closures $\annulus_1,\annulus_2$ of two neighboring
components in $\hat \torus- \torus_0$ are essential annuli
in $M_1,M_2$, respectively. By the vertical-horizontal theorem \cite[Corollary $5.7$]{Joh:79},
one can isotope the fibration on $M_1,M_2$ so that
$\annulus_1,\annulus_2$ are vertical, 
but this implies $\hat M$ 
is Seifert fibered, a contradiction. 
Therefore $\hat \torus\cap \torus_0=\emptyset$ and hence 
$\hat \torus, \torus_0$ are isotopic. 
It may thus be assumed that $\hat\torus=\torus_0$; 
let $M_1$ be the component containing $\Compl\HK$.


Suppose $\Compl\HK$ admits a non-separating essential annulus $\bar \annulus$ disjoint from $\annulus$. 
Then $\bar \annulus$ is non-separating in $M_1$ 
and furthermore, it is essential in $M_1$ 
by the $\partial$-irreducibility of $M_1$, 
contradicting the fact that no essential non-separating annulus exists in a Seifert fiber space over the disk with two exceptional fibers.    
\end{proof}

\begin{lemma}\label{lm:cano_ann_stick_type}
If the characteristic diagram of 
the exterior $\Compl\HK$ of $\pair$
is \raisebox{-.1\height}{\includegraphics[scale=.2]{char_diag_stick}},
then its annulus diagram is \raisebox{-.1\height}{\includegraphics[scale=.2]{ann_diag_stick}},
for some non-integral $r\in\mathbb{Q}$.
\end{lemma}
\begin{proof}
Let $\annulus$ be the characteristic annulus 
of $\Compl\HK$ and $V\subset\Compl\HK$ 
the solid torus cut off by $\annulus$. Set 
$U:=\overline{\Compl\HK-V}$, and
%the closure of the complement of $V$;
denote by $\pi:U\rightarrow B$ the $I$-bundle structure
over a Klein bottle with one open disk removed. 
By Lemma \ref{lm:typefourone_exclusion}, 
$A$ cannot be of type $4$-$1$ 
since $\Compl\HK$ admits a non-separating annulus.
 

Since $B$ is a Klein bottle with one open disk removed,
there exist two simple loops $l,l'\subset B$ with 
$l\cap l'$ a point and $\pi^{-1}(l)$ an annulus $\annulus_l$ and $\pi^{-1}(l')$ a M\"obius band $\mobius_l'$ such that $U$ is a regular neighborhood of $A\cap M$. In particular, the homology classes $u_a,u_m$
of the cores of $\annulus_l, \mobius_l'$, respectively, generate $H_1(U)$.
Since $\annulus$ is the frontier of 
$U$ in $\Compl\HK$, the image of 
a generator of $H_1(\annulus)$ under the homomorphism $H_1(\annulus)\rightarrow H_1(U)$ is $2u_a$. 
%hence the quotient group of $H_1(U)$ by the image of 
%$H_1(A_c)\rightarrow H_(U)$ has torsion, 
Therefore by Lemma \ref{lm:typethreetwoii_generator}, 
$A$ is of type $3$-$2$i  . 
\end{proof} 

Return to the example $\pairfivetwo$; by Lemma \ref{lm:cano_ann_stick_type}, 
$\annulus_c\subset \Compl{5_2}$ is of type $3$-$2$i. 
Now, to determine
the slope of $\annulus_c$, we recall 
that, if $\disk_c\subset\HK$
is a non-separating disk disjoint from $\partial \annulus_c$, 
then $\annulus_c$ is the cabling annulus of 
%the core $c_w$ 
%of 
the solid torus 
$W:=\HK-\openrnbhd{D_c}$ in $\sphere$. 
Thus to compute the slope of $\annulus_c$, 
it amounts to identifying the knot type of $(\sphere, W)$. 
To identify the knot type of $(\sphere, W)$, 
we need only to search for an essential separating disk $\disk_s\subset\HK$ disjoint from $\partial \annulus_c$ 
since $\disk_s$ would cut $\HK$ 
into two pieces with one being isotopic to $W$ in $\sphere$. 


To find such a $\disk_s$, we let $\annulus^\flat$ be 
the annulus $\rnbhd{\mobius}\cap \HK$, where $\rnbhd{\mobius}$ is 
a regular neighborhood of $\mobius$ in $\Compl\HK$. 
Note that
$\partial \annulus$ meets $\annulus^\flat$ at two arcs, which cut $\annulus^\flat$ 
into two disks $\disk_1,\disk_2$ (see Fig.\ \ref{fig:boundary}).  
Since $\annulus_c$ is 
the frontier of a regular neighborhood of 
$\annulus\cup \mobius$, the loop $l:=\overline{\partial \annulus-\disk_i\cup \disk_i-\annulus}$, $i=1$ or $2$, is parallel to components of $\partial \annulus_c$. 

Consider now the disk
$\disk_a$ bounded by the meridian indicated in Fig.\ \ref{fig:meridian}, and observe 
that $\disk_a\cap\partial \annulus$ is a point and
$\disk_a\cap \partial \mobius=\emptyset$. 
The component $\disk_s$ of the frontier of 
a regular neighborhood of $\disk_a\cup l$ in $\HK$
not parallel to $\disk_a$ is then the separating disk
searched for. 
 

\begin{figure}[h]
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{boundary}
\caption{$A, D_1$ and $l$.}
\label{fig:boundary}
\end{subfigure} 
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{meridian}
\caption{Dual meridian.}
\label{fig:meridian}
\end{subfigure} 
\end{figure} 

To visualize $l$, we observe that the boundary components
of $\partial \annulus$ and $\disk_1$ are embedded in $\partial \HK$ as depicted in Fig.\ \ref{fig:boundary_A_M1prime}, and therefore $l$ is the loop in $\partial\HK$ shown in Fig.\ \ref{fig:boundary_Ac}. 

\begin{figure}[h]
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{difference_bA_bD1}
\caption{$\partial \annulus, \disk_1$ in $\partial\HK$.}
\label{fig:boundary_A_M1prime}
\end{subfigure} 
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{boundary_Ac}
\caption{$l$ in $\partial\HK$.}
\label{fig:boundary_Ac}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{DDa_lprime}
\caption{$\disk_a^\pm$ and $l'$.}
\label{fig:DDa_lprime}
\end{subfigure} 
\begin{subfigure}{.45\linewidth}
\center
\includegraphics[scale=.1]{Kl_fivetwo}
\caption{$K_l$ in $\pairfivetwo$.}
\label{fig:Kl_fivetwo}
\end{subfigure} 
\end{figure} 

Let $\disk_a^+, \disk_a^-$ the frontier of $\rnbhd{\disk_a}$ in $\HK$.
Then the disk $\disk_s$ is isotopic in $\HK$ 
to the disk component of 
the frontier of a regular neighborhood of $K_l:=\disk_a^+\cup \disk_a^-\cup l'$ not parallel $\disk_a^\pm$, where $l':=l-\openrnbhd{\disk_a}$. Isotope $K_l$ so that it is as shown in Fig.\ \ref{fig:DDa_lprime}.
For the sake of simplicity, we encode the relation of $K_l$
with $\HK$ in Fig.\ \ref{fig:Kl_fivetwo}. 
Isotope $\pairfivetwo$ in $\sphere$ based on how $l'$ is twisted around $\HK$. Then after a series of isotopies indicated in Figs.\ \ref{fig:deformation1}, \ref{fig:deformation2} and \ref{fig:deformation3}, 
we end up with  
the handlebody-knot in Fig.\ \ref{fig:disk_Ds}, 
a simpler expression for the separating disk $\disk_s$.

It is then not difficult to see 
$\pairfiveone$ can be thought of 
as a regular neighborhood of 
$(4,3)$-torus $K_{4,3}$ 
with a $1$-handle attached as highlighted in Figs.\ \ref{fig:torus_knot_form1} and \ref{fig:torus_knot_form2}.
Hence the slope of $\disk_c$ is $\frac{4}{3}$, and 
we have thus proved the following.
\begin{theorem}\label{teo:hkfivetwo_ann_diag}
The annulus diagram of $\pairfivetwo$ is 
\raisebox{-.2\height}{\includegraphics[scale=.2]{hkfivetwo_ann_diag}}.
\end{theorem}
 

\begin{figure}[h]
\begin{subfigure}{.32\linewidth}
\center
\includegraphics[scale=.07]{deformation1}
\caption{Deform $\pairfivetwo$---I.}
\label{fig:deformation1}
\end{subfigure} 
\begin{subfigure}{.32\linewidth}
\center
\includegraphics[scale=.07]{deformation2}
\caption{Deform $\pairfivetwo$---II.}
\label{fig:deformation2}
\end{subfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.32\linewidth}
\center
\includegraphics[scale=.07]{deformation3}
\caption{Deform $\pairfivetwo$---III.}
\label{fig:deformation3}
\end{subfigure} 
\begin{subfigure}{.32\linewidth}
\center
\includegraphics[scale=.07]{deformation_end}
\caption{Disk $D_s$.}
\label{fig:disk_Ds}
\end{subfigure} 
\begin{subfigure}{.32\linewidth}
\center
\includegraphics[scale=.07]{torus_knot_form1}
\caption{Torus knot with an arc---I.}
\label{fig:torus_knot_form1}
\end{subfigure}
\begin{subfigure}{.32\linewidth}
\center
\includegraphics[scale=.07]{torus_knot_form2}
\caption{Torus knot with an arc---II.}
\label{fig:torus_knot_form2}
\end{subfigure}
\end{figure}


 
Note that by \cite[Theorem $1.2$]{Wan:22p}
the annulus diagram of $\pair$ 
is \raisebox{-.2\height}{\includegraphics[scale=.2]{char_diag_stick}} if and only if 
its exterior $\Compl\HK$ admits infinitely many
essential annuli. All essential annuli in $\Compl\HK$
but one are separating with the unique non-separating one being necessarily 
of type $3$-$3$ by \cite[Theorem $1.5$]{Wan:22p}, and all essential annuli but one 
is non-characteristic with the characteristic one being of 
type $3$-$2$i by Lemma \ref{lm:cano_ann_stick_type}. 
It is thus interesting to consider the following question for such a $\pair$.
\begin{question}
What are the types of the non-separating non-characteristic annuli in $\Compl\HK$?
\end{question}
\begin{question}
Are there any constraints on the slope pair of 
the non-separating annulus or on the slope
of the characteristic annulus in $\Compl\HK$?
\end{question}
 
%\subsection{Handlebody-knot family}
%the twist construction
 

%examples:Motto, LeeLee1, LeeLee2, LeeLee1'
%the three plus two infinite handlebody-knot families



 





